BOston Neonatal Brain Injury Data for Hypoxic Ischemic Encephalopathy (BONBID-HIE): II. 2-year Neurocognitive Outcome and NICU Outcome

Hypoxic Ischemic Encephalopathy (HIE) affects approximately 1-5/1000 newborns globally and leads to adverse neurocognitive outcomes in 30% to 50% of cases by two years of age. Despite therapeutic advances with Therapeutic Hypothermia (TH), prognosis remains challenging, highlighting the need for improved biomarkers. This paper introduces the second release of the Boston Neonatal Brain Injury Dataset for Hypoxic-Ischemic Encephalopathy (BONBID-HIE), an open-source, comprehensive MRI and clinical dataset featuring 237 patients, including NICU outcomes and 2-year neurocognitive outcomes from Massachusetts General Hospital and Boston Children's Hospital.

==> figures/vis_case.tex <==
\begin{figure}[!h]
\centering   

\begin{minipage}{\textwidth}
\centering
\makebox[0.15\linewidth]{\makecell{ADC}} 
\makebox[0.15\linewidth]
{\makecell{\shortstack{Expert\\ Annotations}}} 
\hspace{2mm}
\makebox[0.15\linewidth]{\makecell{ADC}} 
\makebox[0.15\linewidth]
{\makecell{\shortstack{Expert\\ Annotations}}}  
\hspace{2mm}
\makebox[0.15\linewidth]{\makecell{ADC}} 
\makebox[0.15\linewidth]
{\makecell{\shortstack{Expert\\ Annotations}}} 
\end{minipage}
% {\includegraphics[width=0.15\linewidth]{figures/vis/HIE_001/adc.png}}
% {\includegraphics[width=0.15\linewidth]{figures/vis/HIE_001/gt.png}}
% \hspace{2mm}
% {\includegraphics[width=0.15\textwidth]{figures/vis/HIE_348/adc.png}}
% {\includegraphics[width=0.15\textwidth]{figures/vis/HIE_348/gt.png}}
% \hspace{2mm}
% {\includegraphics[width=0.15\textwidth]{figures/vis/HIE_393/adc.png}}
% {\includegraphics[width=0.15\textwidth]{figures/vis/HIE_393/gt.png}}

\begin{minipage}{\textwidth}
\centering
{\includegraphics[width=0.3\linewidth]{figures/vis/001.png}}
\hspace{2mm}
{\includegraphics[width=0.3\textwidth]{figures/vis/070.png}}
\hspace{2mm}
{\includegraphics[width=0.3\textwidth]{figures/vis/302.png}}
\end{minipage}




\begin{minipage}{\textwidth}
\centering
\makebox[0.3\linewidth]{\makecell{Patient 001\\Brain injured~$0.82\%$}} 
\hspace{2mm}
\makebox[0.3\linewidth]{\makecell{Patient 070\\Brain injured~$0.65\%$}} 
\hspace{2mm}
\makebox[0.3\linewidth]{\makecell{Patient 302\\ Brain injured~$4.15\%$}} 
\end{minipage}
\caption{Lesions associated to hypoxic ischemic encephalopathy (HIE) are typically diffuse (i.e., multi-focal) and small. Here we show two representative images for 3 HIE patients. For each patient, in the left panel: apparent diffusion coefficient (ADC) maps that are clinically used to identify HIE lesions; in the right panel: manually-annotated lesions (shown in pink) overlaid on the ADC map. We listed the percentage of the whole brain volume being injured at the bottom (i.e., lesion volume divided by the whole brain volume).}\label{fig:viscase}

\end{figure}
%Lesion of HIE on basal ganglia region in brains. 



    
     

==> tables/cohort_bch.tex <==
\begin{table}[!b]
\centering
\caption{Cohort characteristics in BCH (N=93)}\label{tab:cohort}
\resizebox{0.9\linewidth}{!}
{
\begin{tabular}{l l l }
%Variants & \\
\toprule
\textbf{A. Demographics and Clinical Characteristics}\\
\midrule
\bf{Maternal Information}\\
\midrule
Maternal age at delivery (years) &$31.43 \pm 5.01$&N=93\\
Race& \shortstack{White (68), Black or African American (6), Hispanic or Latino (2), \\ Multi Race (0), Unknown (9), Other (8)}& N=93 \\
Delivery& C-section (58), Vaginal (35)& N=93\\
Antepartum hemorrhage & Yes (12), No (81) & N=93 \\
Thyroid dysfunction & Yes (7), No (86) & N=93\\
Pre-eclampsia & Yes (1), No (92) & N=93\\
Fetal decels& Yes (72), No (21) & N=93\\
Shoulder dystocia & Yes (3), No (90) & N=93\\
Chorioamnionitis & Yes (4), No (89) & N=93\\
Emergency c-section & Yes (51), No (42) & N=93\\
\midrule
\bf{Neonatal Information}\\
\midrule
Age at scan (days) & $2.98\pm2.51$& N=93 \\
%(median(IQR))
Gestational age at birth (weeks)&$39.06\pm1.88$&N=93\\
Birth weight (g)&$3261.41\pm592.26$&N=92\\
Infant head circumference (cm)&$34.45 \pm 1.88$&N=73\\
Sex & Male (58), Female (35) & N=93\\
1-minute APGAR scores &$1.95 \pm 1.88$&N=92\\
5-minute APGAR scores &$3.90 \pm 2.28$&N=92\\
10-minute APGAR scores&$5.05 \pm 2.34$&N=79\\
Lowest pH value in umbilical cord  & $6.98\pm0.24$& N=85\\
Therapeutic hypothermia before MRI? & Yes (77), No (16)& N=93\\
Endotracheal tube (ETT) in NICU & Yes (81), No (12) & N=93\\
Total parenteral nutrition (TPN) in NICU & Yes (91), No (2) & N=93\\
Seizures NICU & Yes (45), No (48) & N=93\\
Length of stay in NICU (days) & $11.46\pm9.48$& N=93\\
\midrule
\textbf{B. NICU Outcome}&Deceased (9),
Survived (84)&N=93\\
\midrule
\textbf{C. 2-year Neurocognitive Outcome}&
Adverse (56), Normal (37)& N=93\\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/cohort_mgh.tex <==
\begin{table}[!b]
\centering
\caption{Cohort characteristics (N=144) in MGH}\label{tab:cohort}
\resizebox{0.9\linewidth}{!}
{
\begin{tabular}{l l l }
%Variants & \\
\toprule
\textbf{A. Demographics and Clinical Characteristics}\\
\midrule
\bf{Maternal Information}\\
\midrule
Maternal age at delivery (years) &$29.58 \pm 6.51$&N=144\\
Race& \shortstack{White (49), Black or African American (7), Hispanic or Latino (16), \\ Multi Race (5), Unknown (60), Other (7)}& N=144 \\
Delivery& C-section (85), Vaginal (55)& N=144\\
Antepartum hemorrhage & Yes (31), No (113) & N=144 \\
Thyroid dysfunction & Yes (5), No (135) & N=144\\
Pre-eclampsia & Yes (9), No (135) & N=144\\
Fetal decels& Yes (81), No (63) & N=144\\
Shoulder dystocia & Yes (8), No (136) & N=144\\
Chorioamnionitis & Yes (22), No (117) & N=144\\
Emergency c-section & Yes (76), No (67) & N=143\\
\midrule
\bf{Neonatal Information}\\
\midrule
Age at scan (days) & $3.81\pm2.26$& N=139 \\
%(median(IQR))
Gestational age at birth (weeks)&$39.09\pm1.97$&N=144\\
Birth weight (g)&$3314.92\pm610.33$&N=144\\
Infant head circumference (cm)&$34.13 \pm 1.52$&N=92\\
Sex & Male (79), Female (65) & N=144\\
1-minute APGAR scores &$1.85 \pm 1.75$&N=144\\
5-minute APGAR scores &$4.03 \pm 2.39$&N=143\\
10-minute APGAR scores&$5.02 \pm 2.37$&N=128\\
Lowest pH value in umbilical cord  & $7.00\pm0.22$& N=140\\
Therapeutic hypothermia before MRI? & Yes (94), No (50)& N=144\\
Endotracheal tube (ETT) in NICU & Yes (87), No (47) & N=134\\
Total parenteral nutrition (TPN) in NICU & Yes (118), No (25) & N=143\\
Seizures NICU & Yes (70), No (74) & N=144\\
Length of stay in NICU (days) & $11.82\pm10.09$& N=144\\
\midrule
\textbf{B. NICU Outcome}&Deceased (24),
Survived (120)&N=144\\
\midrule
\textbf{C. 2-year Neurocognitive Outcome}&
Adverse (47), Normal (67)& N=114\\
\bottomrule
\end{tabular}
}
\end{table}

